LeapsAndBounds: A Method for Approximately Optimal Algorithm Configuration

We consider the problem of configuring general-purpose solvers to run efficiently on problem instances drawn from an unknown distribution. The goal of the configurator is to find a configuration that runs fast on average on most instances, and do so with the least amount of total work. It can run a chosen solver on a random instance until the solver finishes or a timeout is reached. We propose LeapsAndBounds, an algorithm that tests configurations on randomly selected problem instances for longer and longer time. We prove that the capped expected runtime of the configuration returned by LeapsAndBounds is close to the optimal expected runtime, while our algorithm's running time is near-optimal. Our results show that LeapsAndBounds is more efficient than the recent algorithm of Kleinberg et al. (2017), which, to our knowledge, is the only other algorithm configuration method with non-trivial theoretical guarantees. Experimental results on configuring a public SAT solver on a new benchmark dataset also stand witness to the superiority of our method.

==> header.tex <==
%!TEX root =  paper.tex
%\usepackage[T1]{fontenc}
%\usepackage[utf8]{inputenc}
\usepackage{lmodern}
\usepackage[english]{babel}
\usepackage{latexsym}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{enumitem} % we prefer enumitem because of its margin adjustment caps
\usepackage{bm}
\usepackage{datetime}
\usepackage[table,xcdraw]{xcolor}

\renewcommand\labelitemi{--}

% \usepackage{enumerate}
\usepackage{accents}
\usepackage{tikz}
\usepackage{listings}
\usepackage{mdframed}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{dsfont}
\usepackage{color}
\usepackage{colortbl}
\usepackage{pifont}
\usepackage[bf,font=small,singlelinecheck=off]{caption}
\usepackage[textsize=tiny]{todonotes}
%\usepackage[disable]{todonotes}
\usepackage{microtype} % improved spacing between words for easier reading
\usepackage{float}
\usepackage{xfrac} % sfrac
\usepackage{xspace}
%\usepackage[ruled]{algorithm2e}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Various info-block environments based on https://github.com/rstudio/bookdown
% In particular, the following environments are provided:
% 		rmdnote, rmdcaution, rmdimportant, rmdtip, rmdwarning
%
% Here, rmd stands for R-markdown.. Perhaps change this..
\usepackage{framed,color}
%\definecolor{shadecolor}{RGB}{248,248,248}
\definecolor{shadecolor}{RGB}{255,255,255}

\makeatletter
\newenvironment{kframe}{%
\medskip{}
\setlength{\fboxsep}{.8em}
 \def\at@end@of@kframe{}%
 \ifinner\ifhmode%
  \def\at@end@of@kframe{\end{minipage}}%
  \begin{minipage}{\columnwidth}%
 \fi\fi%
 \def\FrameCommand##1{\hskip\@totalleftmargin \hskip-\fboxsep
 \colorbox{shadecolor}{##1}\hskip-\fboxsep
     % There is no \\@totalrightmargin, so:
     \hskip-\linewidth \hskip-\@totalleftmargin \hskip\columnwidth}%
 \MakeFramed {\advance\hsize-\width
   \@totalleftmargin\z@ \linewidth\hsize
   \@setminipage}}%
 {\par\unskip\endMakeFramed%
 \at@end@of@kframe}
\makeatother

%\renewenvironment{Shaded}{\begin{kframe}}{\end{kframe}}
\newenvironment{Shaded}{\begin{kframe}}{\end{kframe}}

\newenvironment{rmdblock}[1]
  {
  \begin{itemize}
  \renewcommand{\labelitemi}{
    \raisebox{-.7\height}[0pt][0pt]{
      {\setkeys{Gin}{width=3em,keepaspectratio}\includegraphics{img/assets/#1}}
    }
  }
  \setlength{\fboxsep}{1em}
  \begin{kframe}
  \item
  }
  {
  \end{kframe}
  \end{itemize}
  }
\newenvironment{rmdnote}
  {\begin{rmdblock}{note}}
  {\end{rmdblock}}
\newenvironment{rmdcaution}
  {\begin{rmdblock}{caution}}
  {\end{rmdblock}}
\newenvironment{rmdimportant}
  {\begin{rmdblock}{important}}
  {\end{rmdblock}}
\newenvironment{rmdtip}
  {\begin{rmdblock}{tip}}
  {\end{rmdblock}}
\newenvironment{rmdwarning}
  {\begin{rmdblock}{warning}}
  {\end{rmdblock}}
\newenvironment{rmdexperiment}
  {\begin{rmdblock}{experiment}}
  {\end{rmdblock}}
\newenvironment{rmdalgorithm}
  {\begin{rmdblock}{algorithm}}
  {\end{rmdblock}}



\usepackage{notes} % importantnote, warningnote, informationnote; we may need to change this as this is pretty ugly
\setlength{\textwd}{1.05\textwidth} % somehow the notes were too narrow


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\makeatletter
\renewcommand{\todo}[2][]{\tikzexternaldisable\@todo[#1]{#2}\tikzexternalenable}
\makeatother

\setlength{\marginparwidth}{13ex}
\newcommand{\todoc}[2][]{\todo[size=\scriptsize,color=blue!20!white,#1]{Csaba: #2}}
\newcommand{\todot}[2][]{\todo[size=\scriptsize,color=red!20!white,#1]{Tor: #2}}

\AtBeginDocument{
  \addtocontents{toc}{\footnotesize}
  \addtocontents{lof}{\footnotesize}
}


\newcommand{\smallsc}[1]{\text{\scalebox{0.9}{\scshape #1}}}
\usepackage{hyperref}
\hypersetup{
    bookmarks=true,         % show bookmarks bar?
    unicode=false,          % non-Latin characters in AcrobatÕs bookmarks
    pdftoolbar=true,        % show AcrobatÕs toolbar?
    pdfmenubar=true,        % show AcrobatÕs menu?
    pdffitwindow=false,     % window fit to page when opened
    pdfstartview={FitH},    % fits the width of the page to the window
    pdftitle={Bandit Algorithms},    % title
    pdfauthor={Lattimore and Szepesvari},     % author
    pdfsubject={Bandits},   % subject of the document
    pdfcreator={Creator},   % creator of the document
    pdfproducer={Producer}, % producer of the document
    pdfkeywords={keyword1} {key2} {key3}, % list of keywords
    pdfnewwindow=true,      % links in new window
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=blue,          % color of internal links (change box color with linkbordercolor)
    citecolor=blue,        % color of links to bibliography
    filecolor=magenta,      % color of file links
    urlcolor=cyan           % color of external links
}
\usepackage{amsthm}
\usepackage{times}
\usepackage{natbib}
\usepackage{nicefrac}
\usepackage{wrapfig}
\usepackage[capitalize]{cleveref}
\usepackage[nottoc,numbib]{tocbibind}

\iffalse
\usepackage{fancyhdr}
\renewcommand{\chaptermark}[1]{\markboth{#1}{}}
\renewcommand{\sectionmark}[1]{\markright{#1}}
\pagestyle{fancy}
\fancyhf{}
\fancyhead[LE,RO]{\thepage}
\fancyhead[LO]{\itshape\nouppercase{\rightmark}}
\fancyhead[RE]{\itshape\nouppercase{\leftmark}}
\renewcommand{\headrulewidth}{0pt}

\setlength{\headheight}{130pt} 
\fi

%\usepackage[lmargin=1.75in,rmargin=1.75in,bmargin=1in]{geometry}
% why the wide margins?
\usepackage[bmargin=1in]{geometry}
\usepackage[normalem]{ulem}

\iffalse
\usepackage[explicit]{titlesec}
\titleformat{\chapter}[display]
{\normalfont\Large\scshape}{\centering\uline{\chaptertitlename\ \thechapter}}{20pt}{\centering \Large #1}
\titleformat{\section}[hang]
{\normalfont\normalsize\scshape}{\uline{\thesection}}{10pt}{\normalsize\scshape\uline{#1}}
\titlespacing*{\section}{0pt}{10pt}{5pt}
\fi

\iffalse
\newenvironment{tip}[1][Tip]{
\tikzset{external/export next=false}
\noindent
\ignorespaces
\begin{center}
\begin{tikzpicture}
%\node[inner sep=10pt,text width=0.9\textwidth,draw=gray!20!white,line width=10pt,fill=gray!20!white,anchor=south] (title) at (0,-10pt) {\textbf{#1}};
\node[inner sep=10pt,text width=0.9\textwidth,line width=5pt,draw=gray!40!white,anchor=north] at (0,0) \bgroup \begin{minipage}{\textwidth} \textbf{#1} \par \noindent}{\end{minipage}\egroup;
\end{tikzpicture}
\end{center}
\par\noindent\ignorespacesafterend}
\fi

\newenvironment{tip}[1][Tip]{
\tikzset{external/export next=false}
\par\noindent\tikz{\draw[line width=1pt] (0,0) -- (\linewidth, 0);}
\par\noindent \textbf{#1}\,\, \noindent
}{
\tikzset{external/export next=false}
\par\noindent\tikz{\draw[line width=1pt] (0,0) -- (\linewidth, 0);} \par}


\usepgfplotslibrary{external}
\tikzexternalize[prefix=tikz/]
\tikzset{external/export=true}

\setcounter{tocdepth}{0}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% HYPHENATION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pretolerance=5000
\tolerance=9000
\emergencystretch=0pt
\righthyphenmin=4
\lefthyphenmin=4

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}

\newtheorem{exercise}{Exercise}[section]
\theoremstyle{remark}

\bibliographystyle{plainnat}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

%\newcommand{\lefteqn}[1]{\rlap{\displaystyle{#1}}}
\newcommand{\E}{\mathbb E}
\newcommand{\Var}{\mathbb V}
\newcommand{\V}{\mathbb V}
\newcommand{\Kurt}{\operatorname{Kurt}}
\newcommand{\Supp}{\operatorname{Supp}}
\newcommand{\vol}{\mathrm{vol}}
\newcommand{\diam}{\mathrm{diam}}
\newcommand{\dom}{\mathrm{dom}}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\ind}{\mathbb{I}}
\newcommand{\inner}[1]{\left\langle #1 \right\rangle}
\newcommand{\shortinner}[1]{\langle #1 \rangle}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\sgn}{\operatorname{sign}}
\newcommand{\KL}{\operatorname{D}}
\newcommand{\laspan}{\operatorname{span}}
\newcommand{\EE}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\Et}[1]{\mathbb{E}_t\!\left[#1\right]}
\newcommand{\VV}[1]{\mathbb{V}\left[#1\right]}
\newcommand{\Vt}[1]{\mathbb{V}_t\!\left[#1\right]}
\newcommand{\Prob}[1]{\mathbb{P}\left(#1\right)}
\renewcommand{\P}[1]{\mathbb{P}\left(#1\right)}
\newcommand{\Probng}[1]{\mathbb{P}(#1)}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\one}[1]{\mathbb{I}\left\{#1\right\}}
\newcommand{\erf}{\operatorname{erf}}
\newcommand{\erfc}{\operatorname{erfc}}
\newcommand{\ip}[1]{\langle #1 \rangle}
\newcommand{\bip}[1]{\left\langle #1 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\grnorm}[1]{\left\|#1\right\|}
\newcommand{\eps}{\varepsilon}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\BR}{\operatorname{BR}}
\newcommand{\RS}{R^{\text{\tiny \textsc{simple}}}}
\newcommand{\FP}{\operatorname{FP}}
\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\co}{co}
\DeclareMathOperator{\clip}{clip}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cU}{\mathcal{U}}

\newcommand{\bbP}{\mathbb P}
\newcommand{\bbQ}{\mathbb Q}

\newcommand{\Beta}{\operatorname{Beta}}

\renewcommand{\epsilon}{\varepsilon}
\newcommand{\ceil}[1]{\left\lceil {#1} \right\rceil}
\newcommand{\floor}[1]{\left\lfloor {#1} \right\rfloor}
\newcommand{\Ctx}{\mathrm{C}}
\newcommand{\UCB}{\mathrm{UCB}}
\newcommand{\LCB}{\mathrm{LCB}}
\newcommand{\subG}{\mathrm{subG}}
\newcommand{\defeq}{\doteq}
\newcommand{\hint}[1]{(\textbf{Hint:} #1\xspace)}
\newcommand{\Play}{\text{\sc Play}\xspace}
\newcommand{\DoNothing}{\text{\sc DoNothing}\xspace}
\newcommand{\iid}{i.i.d.\xspace}
% PGFPLOTS STUFF 

\usepgfplotslibrary{statistics}

\definecolor{PlotColor1}{HTML}{30A2DA}
\definecolor{PlotColor2}{HTML}{6D904F}
\definecolor{PlotColor3}{HTML}{E5AE38}
\definecolor{PlotColor4}{HTML}{FC4F30}
\definecolor{PlotColor5}{HTML}{8b8b8b}
\definecolor{PlotColor6}{HTML}{000000}

\pgfplotscreateplotcyclelist{PlotsCycleList}{
  {smooth,PlotColor1,ultra thick},
  {smooth,PlotColor2,ultra thick},
  {smooth,PlotColor3,ultra thick},
  {smooth,PlotColor4,ultra thick},
  {smooth,PlotColor5,ultra thick},
  {smooth,PlotColor6,ultra thick},
}

\pgfplotsset{every axis/.append style={legend pos=outer north east,legend cell align={left},cycle list name=PlotsCycleList}}






%\iffalse


% Mass generation of bold, blackboard bold, caligraphic, and "vector" symbols:
\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}

% \bA, \bB, ...
\def\ddef#1{\expandafter\def\csname b#1\endcsname{\ensuremath{\mathbf{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

% \bbA, \bbB, ...
\def\ddef#1{\expandafter\def\csname bb#1\endcsname{\ensuremath{\mathbb{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

% \cA, \cB, ...
\def\ddef#1{\expandafter\def\csname c#1\endcsname{\ensuremath{\mathcal{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

% \vA, \vB, ..., \va, \vb, ...
\def\ddef#1{\expandafter\def\csname v#1\endcsname{\ensuremath{\boldsymbol{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz\ddefloop

% \valpha, \vbeta, ...,  \vGamma, \vDelta, ...,
\def\ddef#1{\expandafter\def\csname v#1\endcsname{\ensuremath{\boldsymbol{\csname #1\endcsname}}}}
\ddefloop {alpha}{beta}{gamma}{delta}{epsilon}{varepsilon}{zeta}{eta}{theta}{vartheta}{iota}{kappa}{lambda}{mu}{nu}{xi}{pi}{varpi}{rho}{varrho}{sigma}{varsigma}{tau}{upsilon}{phi}{varphi}{chi}{psi}{omega}{Gamma}{Delta}{Theta}{Lambda}{Xi}{Pi}{Sigma}{varSigma}{Upsilon}{Phi}{Psi}{Omega}\ddefloop


%\fi


